How to Learn a New Language? An Efficient Solution for Self-Supervised Learning Models Unseen Languages Adaption in Low-Resource Scenario

The utilization of speech Self-Supervised Learning (SSL) models achieves impressive performance on Automatic Speech Recognition (ASR). However, in low-resource language ASR, they encounter the domain mismatch problem between pre-trained and low-resource languages. Typical solutions like fine-tuning the SSL model suffer from high computation costs while using frozen SSL models as feature extractors comes with poor performance. To handle these issues, we extend a conventional efficient fine-tuning scheme based on the adapter. We add an extra intermediate adaptation to warm up the adapter and downstream model initialization. Remarkably, we update only 1-5% of the total model parameters to achieve the adaptation. Experimental results on the ML-SUPERB dataset show that our solution outperforms conventional efficient fine-tuning. It achieves up to a 28% relative improvement in the Character/Phoneme error rate when adapting to unseen languages.

==> tables/MLSUPERB.tex <==
\scalebox{0.7}{\begin{tabular}{c|cccc}
\toprule
\multirow{3}{*}{SSL} & \multicolumn{4}{c}{CER/PER}                                                               \\ \cmidrule{2-5} 
                     & \multicolumn{2}{c|}{Mono}                              & \multicolumn{2}{c}{Reserve}      \\ \cmidrule{2-5} 
                     & \multicolumn{1}{c|}{10min} & \multicolumn{1}{c|}{1h}   & \multicolumn{1}{c|}{10min} & 1h   \\ \midrule
HuBERT               & \multicolumn{1}{c|}{42.8}  & \multicolumn{1}{c|}{35.3} & \multicolumn{1}{c|}{39.6}  & 31.3 \\ \midrule
mHuBERT              & \multicolumn{1}{c|}{41.0}    & \multicolumn{1}{c|}{33.0}   & \multicolumn{1}{c|}{37.4}  & 29.3 \\ \midrule
XLSR-128             & \multicolumn{1}{c|}{39.7}  & \multicolumn{1}{c|}{30.6} & \multicolumn{1}{c|}{32.1}  & 22.8 \\ \bottomrule

\end{tabular}}

==> tables/Mono_Reserve_cer.tex <==
\resizebox{\linewidth}{4cm}
{\begin{threeparttable}

\begin{tabular}{l|l|cccc}
% {p{13mm}|p{19mm}|p{6mm}p{6mm}p{6mm}p{6mm}}
\toprule 
\multicolumn{1}{c|}{\multirow{3}{*}{SSL}} & \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{Our (pink) \&\\Baselines}}} & \multicolumn{4}{c}{CER/PER $\downarrow$}\\ \cline{3-6} 
                         &                                & \multicolumn{2}{c|}{Seen Set}                       & \multicolumn{2}{c}{Unseen Set}  \\ \cline{3-6} 
                         &                                & 10min & \multicolumn{1}{l|}{1h} &10min & 1h \\ \midrule
                         \midrule
\multirow{6}{*}{\shortstack[l]{ HuBERT \\ \raggedright (95M)}} 
& \cellcolor{full}Full-FT & \multicolumn{1}{l}{\cellcolor{full}42.4}  & \multicolumn{1}{l|}{\cellcolor{full}29.2}& \cellcolor{full}25.7  & \multicolumn{1}{l}{\cellcolor{full}\textbf{18.0}}\\
                        & Freeze-FT & \multicolumn{1}{l}{42.8}  & \multicolumn{1}{l|}{35.3}& 30.4  & \multicolumn{1}{l}{22.2}\\
                         & PEFT & \multicolumn{1}{l}{39.6}  & \multicolumn{1}{l|}{31.3}& 28.9  & \multicolumn{1}{l}{20.6}\\    
                         & $\mathcal{S}$\&$\mathcal{T}$-MTL & \multicolumn{1}{l}{43.3}  & \multicolumn{1}{l|}{42.8} & {30.9}  & \multicolumn{1}{l}{23.4} \\   
                         & \cellcolor{FOMAML}IA-MAML & \multicolumn{1}{l}{\cellcolor{FOMAML}35.9}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}29.3}  & {\cellcolor{FOMAML}26.2} & \cellcolor{FOMAML}20.4  \\  
                         & \cellcolor{FOMAML}IA-MTL & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{34.8}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{28.9}} & {\cellcolor{FOMAML}\textbf{24.6}}  & \cellcolor{FOMAML}19.6 \\ \midrule
\multirow{6}{*}{\shortstack[l]{mHuBERT \\ \raggedright (95M)}} 
& \cellcolor{full}Full-FT & \multicolumn{1}{l}{\cellcolor{full}39.8}  & \multicolumn{1}{l|}{\cellcolor{full}28.6}& \cellcolor{full}24.5  & \multicolumn{1}{l}{\cellcolor{full}18.1}\\
                        & Freeze-FT & \multicolumn{1}{l}{41.0}  & \multicolumn{1}{l|}{33.0}& 29.1  & \multicolumn{1}{l}{22.0}\\
                        & PEFT & \multicolumn{1}{l}{37.4}  & \multicolumn{1}{l|}{29.3}  & {27.5}  & 19.6 \\   
                        & $\mathcal{S}$\&$\mathcal{T}$-MTL & \multicolumn{1}{l}{40.7}  & \multicolumn{1}{l|}{41.1}  & {29.5}  & 22.5\\  
                         & \cellcolor{FOMAML}IA-MAML & \multicolumn{1}{l}{\cellcolor{FOMAML}34.3}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}28.3}   & {\cellcolor{FOMAML}25.8}  & \cellcolor{FOMAML}\textbf{17.1} \\    
                         & \cellcolor{FOMAML}IA-MTL & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{32.6}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{27.2}} & {\cellcolor{FOMAML}\textbf{24.1}}  & \cellcolor{FOMAML}19.6 \\
                         \bottomrule \toprule
                         
\multirow{6}{*}{\shortstack[l]{XLSR-128 \\ \raggedright (317M)}} 
& \cellcolor{full}Full-FT & \multicolumn{1}{l}{\cellcolor{full}27.6}  & \multicolumn{1}{l|}{\cellcolor{full}\textbf{18.3}}& \cellcolor{full}19.3  & \multicolumn{1}{l}{\cellcolor{full}13.5}\\
                         & Freeze-FT & \multicolumn{1}{l}{39.7}  & \multicolumn{1}{l|}{30.6}& 29.8  & \multicolumn{1}{l}{21.5}\\
                         & PEFT & \multicolumn{1}{l}{32.1}  & \multicolumn{1}{l|}{22.8}  & {25.5}  & 16.6  \\    
                         & $\mathcal{S}$\&$\mathcal{T}$-MTL & \multicolumn{1}{l}{51.6}  & \multicolumn{1}{l|}{53.0}  & {20.7}  & 14.6  \\    
                         & \cellcolor{FOMAML}IA-MAML & \multicolumn{1}{l}{\cellcolor{FOMAML}26.4}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}20.0}  & {\cellcolor{FOMAML}21.4}  & \cellcolor{FOMAML}13.6  \\ 
                         &  \cellcolor{FOMAML}IA-MTL & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{24.1}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}19.1}  & {\cellcolor{FOMAML}\textbf{18.3}}  &  {\cellcolor{FOMAML}\textbf{13.2}} \\
 \bottomrule
\end{tabular}
\end{threeparttable}}
% }

==> tables/Mono_track.tex <==
\scalebox{0.60}{\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{3}{*}{SSL}     & \multirow{3}{*}{Priming Algorithm} & \multicolumn{4}{c|}{CER}                                                               & \multicolumn{4}{c}{STD}                                                                   \\ \cline{3-10} 
                         &                                    & \multicolumn{2}{c|}{w/o Adapter}                       & \multicolumn{2}{c|}{w Adapter}    & \multicolumn{2}{c|}{w/o Adapter}                       & \multicolumn{2}{c}{w Adapter}    \\ \cline{3-10} 
                         &                                    & \multicolumn{1}{c|}{10min} & \multicolumn{1}{c|}{1h}   & \multicolumn{1}{c|}{10min} & 1h   & \multicolumn{1}{c|}{10min} & \multicolumn{1}{c|}{1h}   & \multicolumn{1}{c|}{10min} & 1h   \\ \midrule
\multirow{4}{*}{Hubert}  & Directly Fine-tuning               & \multicolumn{1}{c|}{42.8}  & \multicolumn{1}{c|}{35.3} & \multicolumn{1}{c|}{39.6}  & 31.3 & \multicolumn{1}{c|}{11.2}  & \multicolumn{1}{c|}{10.7} & \multicolumn{1}{c|}{12.3}  & 11.2 \\  
                         & Single-Stage MTL                   & \multicolumn{1}{c|}{60.1}  & \multicolumn{1}{c|}{61}   & \multicolumn{1}{c|}{43.3}  & 42.8 & \multicolumn{1}{c|}{13.7}  & \multicolumn{1}{c|}{13.4} & \multicolumn{1}{c|}{13.3}  & 12.7 \\   
                         & \rowcolor{FOMAML}MAML & \multicolumn{1}{c|}{40.6}  & \multicolumn{1}{c|}{33}   & \multicolumn{1}{c|}{36.8}  & 30.1 & \multicolumn{1}{c|}{13.3}  & \multicolumn{1}{c|}{11.9} & \multicolumn{1}{c|}{12.1}  & 11.3 \\   
                         & \rowcolor{MTL}MTL                                & \multicolumn  {1}{c|}{\textbf{38.9}}  & \multicolumn{1}{c|}{\textbf{31.4}} & \multicolumn{1}{c|}{\textbf{34.8}}  & \textbf{28.9} & \multicolumn{1}{c|}{13.3}  & \multicolumn{1}{c|}{12}   & \multicolumn{1}{c|}{11.5}  & 10.9 \\ \midrule
\multirow{4}{*}{mHubert} & Directly Fine-tuning               & \multicolumn{1}{c|}{41}    & \multicolumn{1}{c|}{33}   & \multicolumn{1}{c|}{37.4}  & 29.3 & \multicolumn{1}{c|}{10}    & \multicolumn{1}{c|}{9.9}  & \multicolumn{1}{c|}{11.1}  & 10.5 \\   
                         & Single-Stage MTL                   & \multicolumn{1}{c|}{41.8}  & \multicolumn{1}{c|}{42.5} & \multicolumn{1}{c|}{40.7}  & 41.1 & \multicolumn{1}{c|}{12.3}  & \multicolumn{1}{c|}{12.7} & \multicolumn{1}{c|}{14.7}  & 15.4 \\   
                         & \rowcolor{FOMAML}MAML                             & \multicolumn{1}{c|}{36.7}  & \multicolumn{1}{c|}{30.4} & \multicolumn{1}{c|}{34.3}  & 28.3 & \multicolumn{1}{c|}{10.8}  & \multicolumn{1}{c|}{10.7} & \multicolumn{1}{c|}{10.3}  & 10.7 \\   
                         & \rowcolor{MTL}MTL                                & \multicolumn{1}{c|}{\textbf{34}}    & \multicolumn{1}{c|}{\textbf{28.1}} & \multicolumn{1}{c|}{\textbf{32.6}}  & \textbf{27.2} & \multicolumn{1}{c|}{10.5}  & \multicolumn{1}{c|}{10.5} & \multicolumn{1}{c|}{10.6}  & 10.2 \\
                         \bottomrule \toprule
                         
\multirow{4}{*}{XLSR128} & Directly Fine-tuning               & \multicolumn{1}{c|}{39.7}  & \multicolumn{1}{c|}{30.6} & \multicolumn{1}{c|}{32.1}  & 22.8 & \multicolumn{1}{c|}{13.1}  & \multicolumn{1}{c|}{12}   & \multicolumn{1}{c|}{15.4}  & 13.6 \\   
                         & Single-Stage MTL                   & \multicolumn{1}{c|}{54.1}  & \multicolumn{1}{c|}{56.1} & \multicolumn{1}{c|}{51.6}  & 53   & \multicolumn{1}{c|}{17.4}  & \multicolumn{1}{c|}{16.3} & \multicolumn{1}{c|}{19.7}  & 18.4 \\   
                         &  \rowcolor{FOMAML}MAML                             & \multicolumn{1}{c|}{31.5}  & \multicolumn{1}{c|}{24.9} & \multicolumn{1}{c|}{26.4}  & 20   & \multicolumn{1}{c|}{12.2}  & \multicolumn{1}{c|}{11.5} & \multicolumn{1}{c|}{14}    & 12.5 \\ 
                         &  \rowcolor{MTL}MTL                                & \multicolumn{1}{c|}{\textbf{26.3}}  & \multicolumn{1}{c|}{\textbf{20.3}} & \multicolumn{1}{c|}{\textbf{24.1}}  & \textbf{19.1} & \multicolumn{1}{c|}{13.4}  & \multicolumn{1}{c|}{12.3} & \multicolumn{1}{c|}{13.4}  & 12   \\
 \bottomrule
\end{tabular}


==> tables/Mono_track_10min.tex <==
\scalebox{0.9}{\begin{tabular}{c|c|cccc}
\toprule
\multirow{2}{*}{SSL}     & \multirow{2}{*}{Priming Algorithm} & \multicolumn{2}{c|}{CER}                                                               & \multicolumn{2}{c}{STD}                                                                   \\ \cline{3-6} 
                         &                                    & \multicolumn{1}{c|}{w/o A}                       & \multicolumn{1}{c|}{w A}    & \multicolumn{1}{c|}{w/o A}                       & \multicolumn{1}{c}{w A}    \\ 
                          \midrule
\multirow{4}{*}{Hubert}  & Directly Fine-tuning               & \multicolumn{1}{c|}{42.8}  & \multicolumn{1}{c|}{39.6}  & \multicolumn{1}{c|}{11.2}  & \multicolumn{1}{c|}{12.3}   \\  
                         & Single-Stage MTL                   & \multicolumn{1}{c|}{60.1}  & \multicolumn{1}{c|}{43.3}  & \multicolumn{1}{c|}{13.7}  & \multicolumn{1}{c|}{13.3}  \\   
                         & \rowcolor{FOMAML}FOMAML & \multicolumn{1}{c|}{40.6}  & \multicolumn{1}{c|}{36.8}  & \multicolumn{1}{c|}{13.3}  & \multicolumn{1}{c|}{12.1}  \\   
                         & \rowcolor{MTL}MTL                                & \multicolumn  {1}{c|}{\textbf{38.9}}  & \multicolumn{1}{c|}{\textbf{34.8}}  & \multicolumn{1}{c|}{13.3}  & \multicolumn{1}{c|}{11.5}   \\ \midrule
\multirow{4}{*}{mHubert} & Directly Fine-tuning               & \multicolumn{1}{c|}{41}    & \multicolumn{1}{c|}{37.4} & \multicolumn{1}{c|}{10}    & \multicolumn{1}{c|}{11.1} \\   
                         & Single-Stage MTL                   & \multicolumn{1}{c|}{41.8}  & \multicolumn{1}{c|}{40.7}  & \multicolumn{1}{c|}{12.3}  & \multicolumn{1}{c|}{14.7}  \\   
                         & \rowcolor{FOMAML}FOMAML                             & \multicolumn{1}{c|}{36.7}  & \multicolumn{1}{c|}{34.3}  & \multicolumn{1}{c|}{10.8}  & \multicolumn{1}{c|}{10.3}   \\   
                         & \rowcolor{MTL}MTL                                & \multicolumn{1}{c|}{\textbf{34}}    & \multicolumn{1}{c|}{\textbf{32.6}}  & \multicolumn{1}{c|}{10.5}  & \multicolumn{1}{c|}{10.6}  \\
                         \bottomrule \toprule
                         
\multirow{4}{*}{XLSR128} & Directly Fine-tuning               & \multicolumn{1}{c|}{39.7}  & \multicolumn{1}{c|}{32.1}  & \multicolumn{1}{c|}{13.1}  & \multicolumn{1}{c|}{15.4}  \\   
                         & Single-Stage MTL                   & \multicolumn{1}{c|}{54.1}  & \multicolumn{1}{c|}{51.6}  & \multicolumn{1}{c|}{17.4}  & \multicolumn{1}{c|}{19.7}  \\   
                         &  \rowcolor{FOMAML}FOMAML                             & \multicolumn{1}{c|}{31.5}  & \multicolumn{1}{c|}{26.4}  & \multicolumn{1}{c|}{12.2}  & \multicolumn{1}{c|}{14}    \\ 
                         &  \rowcolor{MTL}MTL                                & \multicolumn{1}{c|}{\textbf{26.3}}  & \multicolumn{1}{c|}{\textbf{24.1}}  & \multicolumn{1}{c|}{13.4}  & \multicolumn{1}{c|}{13.4}  \\
 \bottomrule
\end{tabular}}

==> tables/Mono_track_1h.tex <==
\scalebox{0.9}{\begin{tabular}{c|c|cccc}
\toprule
\multirow{2}[b]{*}{SSL} & \multirow{2}{*}{Priming Algorithm} & \multicolumn{2}{c|}{CER}                                                               & \multicolumn{2}{c}{STD}                                                                   \\ \cline{3-6} 
                         &                                    & \multicolumn{1}{c|}{w/o A}                       & \multicolumn{1}{c|}{w A}    & \multicolumn{1}{c|}{w/o A}                       & \multicolumn{1}{c}{w A}    \\ \midrule
\multirow{4}{*}{Hubert}  & Directly Fine-tuning                 & \multicolumn{1}{c|}{35.3}   & \multicolumn{1}{c|}{31.3}   & \multicolumn{1}{c|}{10.7}  & 11.2 \\  
                         & Single-Stage MTL                   &  \multicolumn{1}{c|}{61}   & \multicolumn{1}{c|}{42.8}   & \multicolumn{1}{c|}{13.4}  & 12.7 \\   
                         & \rowcolor{FOMAML}FOMAML   & \multicolumn{1}{c|}{33}     & \multicolumn{1}{c|}{30.1}  & \multicolumn{1}{c|}{11.9}  & 11.3 \\   
                         & \rowcolor{MTL}MTL                                 & \multicolumn{1}{c|}{\textbf{31.4}} & \multicolumn{1}{c|}{\textbf{28.9}}  & \multicolumn{1}{c|}{12}    & 10.9 \\ \midrule
\multirow{4}{*}{mHubert} & Directly Fine-tuning                   & \multicolumn{1}{c|}{33}    &\multicolumn{1}{c|} {29.3} & \multicolumn{1}{c|}{9.9}  & 10.5 \\   
                         & Single-Stage MTL                   &  \multicolumn{1}{c|}{42.5}   & \multicolumn{1}{c|}{41.1}  & \multicolumn{1}{c|}{12.7} & 15.4 \\   
                         & \rowcolor{FOMAML}FOMAML                              & \multicolumn{1}{c|}{30.4}   & \multicolumn{1}{c|}{28.3}  & \multicolumn{1}{c|}{10.7}& 10.7 \\   
                         & \rowcolor{MTL} MTL                                & \multicolumn{1}{c|}{\textbf{28.1}}   & \multicolumn{1}{c|}{\textbf{27.2}} & \multicolumn{1}{c|}{10.5} & 10.2 \\
                         \bottomrule \toprule
                         
\multirow{4}{*}{XLSR128} & Directly Fine-tuning                & \multicolumn{1}{c|}{30.6}   & \multicolumn{1}{c|}{22.8} & \multicolumn{1}{c|}{12}   & 13.6 \\   
                         & Single-Stage MTL                   & \multicolumn{1}{c|}{56.1}  & \multicolumn{1}{c|}{53}   &  \multicolumn{1}{c|}{16.3}  & 18.4 \\   
                         &  \rowcolor{FOMAML}FOMAML                              & \multicolumn{1}{c|}{24.9}   & \multicolumn{1}{c|}{20}    & \multicolumn{1}{c|}{11.5}  & 12.5 \\ 
                         &  \rowcolor{MTL}MTL                                 & \multicolumn{1}{c|}{\textbf{20.3}} & \multicolumn{1}{c|}{\textbf{19.1}}  & \multicolumn{1}{c|}{12.3}  & 12   \\
 \bottomrule
\end{tabular}}

==> tables/Mono_track_test.tex <==

\begin{threeparttable}

\begin{tabular}{p{13mm}|p{16mm}|p{7mm}p{7mm}p{7mm}p{7mm}}

\toprule 

\multicolumn{1}{c|}{\multirow{3}{*}{SSL}} & \multirow{3}{*}{\shortstack{Priming \\Algorithm}} & \multicolumn{4}{c}{CER/PER}\\ \cline{3-6} 
                         &                                & \multicolumn{2}{c|}{without Adapter}                       & \multicolumn{2}{c}{with Adapter}  \\ \cline{3-6} 
                         &                                & 10m & \multicolumn{1}{l|}{1h} &10m & 1h \\ \midrule
                         \midrule
\multirow{4}{*}{\shortstack[l]{ HuBERT \\ \raggedright (95M)}} & D-F               & 42.8  & \multicolumn{1}{l|}{35.3} & 39.6  & 31.3\\  
                         & 1-MTL                   & 60.1  & \multicolumn{1}{l|}{61.0}   & 43.3  & 42.8\\   
                         & \cellcolor{FOMAML}MAML & \cellcolor{FOMAML}40.6  & \multicolumn{1}{l|}{\cellcolor{FOMAML}33.0}   & \cellcolor{FOMAML}36.8  & \cellcolor{FOMAML}30.1 \\   
                         & \cellcolor{FOMAML}Prime-MTL                                & {\cellcolor{FOMAML}\textbf{38.9}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{31.4}} & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{34.8}}  & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{28.9}} \\ \midrule
\multirow{4}{*}{\shortstack[l]{mHuBERT \\ \raggedright (95M)}} & D-F               & \multicolumn{1}{l}{41.0}    & \multicolumn{1}{l|}{33.0}   & \multicolumn{1}{l}{37.4}  & \multicolumn{1}{l}{29.3}  \\   
                        & 1-MTL                   & \multicolumn{1}{l}{41.8}  & \multicolumn{1}{l|}{42.5} & \multicolumn{1}{l}{40.7}  & \multicolumn{1}{l}{41.1} \\   
                         & \cellcolor{FOMAML}MAML                             & \multicolumn{1}{l}{\cellcolor{FOMAML}36.7}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}30.4} & \multicolumn{1}{l}{\cellcolor{FOMAML}34.3}  & \multicolumn{1}{l}{\cellcolor{FOMAML}28.3}  \\   
                         & \cellcolor{FOMAML}Prime-MTL                                & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{34.0}}    & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{28.1}} & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{32.6}}  & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{27.2}}\\
                         \bottomrule \toprule
                         
\multirow{4}{*}{\shortstack[l]{XLSR-128 \\ \raggedright (317M)}} & D-F               & \multicolumn{1}{l}{39.7}  & \multicolumn{1}{l|}{30.6} & \multicolumn{1}{l}{32.1}  & \multicolumn{1}{l}{22.8}  \\   
                         & 1-MTL                   & \multicolumn{1}{l}{54.1}  & \multicolumn{1}{l|}{56.1} & \multicolumn{1}{l}{51.6}  & \multicolumn{1}{l}{53.0}  \\   
                         & \cellcolor{FOMAML}  MAML                             & \multicolumn{1}{l}{\cellcolor{FOMAML}31.5}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}24.9} & \multicolumn{1}{l}{\cellcolor{FOMAML}26.4}  & \multicolumn{1}{l}{\cellcolor{FOMAML}20.0}   \\ 
                         &  \cellcolor{FOMAML}Prime-MTL                                & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{26.3}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{20.3}} & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{24.1}}  & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{19.1}}  \\
 \bottomrule
\end{tabular}
\end{threeparttable}
% }

==> tables/Reserve_track.tex <==
% \caption{ML-SUPERB Reserve Languages.}
% \scalebox{0.75}{\begin{threeparttable}
% % \caption{ML-SUPERB Reserve Languages.}
% \begin{tabular}{c|c|cccc|cccc}
% \toprule
% \multirow{3}{*}{SSL}     & \multirow{3}{*}{\shortstack{{Priming \\Algorithm}}} & \multicolumn{4}{c|}{CER/PER}                                                               & \multicolumn{4}{c}{STD}                                                                  \\ \cline{3-10} 
%                          &                                    & \multicolumn{2}{c|}{w/o A}                       & \multicolumn{2}{c|}{w/ A}    & \multicolumn{2}{c|}{w/o A}                       & \multicolumn{2}{c}{w/ A}   \\ \cline{3-10} 
%                          &                                    & {10m} & {1h}   & {10m} & 1h   & {10m} & {1h}   & {10m} & 1h  \\ \midrule
%                          \midrule
% \multirow{4}{*}{HuBERT}  & D-F               & {30.4}  & {22.2} & {28.9}  & 20.6 & {16}    & {8.7}  & {15.5}  & 8.5 \\  
%                          & 1-MTL                   & {32}    & {25.3} & {30.9}  & 23.4 & {9.4}   & {8.5}  & {9.6}   & 9.2 \\  
%                           & \rowcolor{FOMAML}MAML & {29.6} & {22}   & {26.2} & 20.4 & {15.2}  & {8.5}  & {10.2}  & 8.5  \\  
%                          & \rowcolor{MTL}Prime-MTL                                & {\textbf{29.3}}  & {\textbf{21.7}} & {\textbf{24.6}}  & \textbf{19.6} & {15.1}  & {8.8}  & {9.7}   & 8.3 \\ \midrule
% \multirow{4}{*}{mHuBERT} & D-F               & {29.1}  & {22}   & {27.5}  & 19.6 & {14.9}  & {10.3} & {14.5}  & 8.7 \\  
%                          & 1-MTL                   & {31.5}  & {25}   & {29.5}  & 22.5 & {9.5}   & {8.1}  & {9.4}   & 8.1 \\  
%                          & \rowcolor{FOMAML}MAML                             & {\textbf{27.7}}  & {22.2} & {25.8}  & \textbf{17.1} & {10.3}  & {10.6} & {16.4}  & 9.9 \\  
%                          & \rowcolor{MTL}Prime-MTL                                & {29.1}  & {\textbf{21.7}}   & {\textbf{24.1}}  & 19.6 & {14.7}  & {9.3}   & {9.7}   & 9.8 \\ \bottomrule \toprule
% \multirow{4}{*}{XLSR-128} & D-F               & {29.8}  & {21.5} & {25.5}  & 16.6 & {19.7}  & {16.4} & {21}    & 16  \\  
%                          & 1-MTL                   & {26.4}  & {19.1} & {20.7}  & 14.6 & {9.1}   & {7.5}  & {7.9}   & 6.1 \\  
%                          & \rowcolor{FOMAML}MAML                             & {25.2}  & {18}   & {21.4}  & 13.6 & {14.4}  & {8}    & {15.7}  & 6.9 \\  
%                          & \rowcolor{MTL}Prime-MTL                                & {\textbf{22.5}}  & {\textbf{17.3}} & {\textbf{18.3}}      &  {\textbf{13.2}}    & {9.2}   & {7.6}  & {8.5}      & 6.8    \\ \bottomrule



% \end{tabular}
% % \begin{tablenotes}[para,flushleft]    
% %         % \footnotesize 
% %         \captionsize
% %         \item Colored rows refer to our priming baselines.\\
% %         \item ``w/o A'' and ``w A'' represents without adapter and with adapter cases.
% %         % \item FOMAML: do first order MAML as priming then fine-tune 
% %         % \item 1-MTL: single step multi-task learning
% %         % \item Prime-MTL: do multi-task learning as priming then fine-tune 
    
% %       \end{tablenotes}     
% %    \caption*{ Colored rows refer to our priming baselines. \\``w/o A'' and ``w/ A'' represents without adapter and with adapter cases.}

% \end{threeparttable}}
% \caption*{ Colored rows refer to our priming baselines. \\``w/o A'' and ``w/ A'' represents without adapter and with adapter cases.}



% \caption{ML-SUPERB Reserve Languages.}

\begin{threeparttable}
    % \captionsetup{justification=raggedright}
    % \captionsetup{font=normal}
    % \caption*{Colored rows refer to our priming baselines.}
% \caption{ML-SUPERB Monolingual Track}
\begin{tabular}{p{13mm}|p{16mm}|p{7mm}p{7mm}p{7mm}p{7mm}}
% \begin{tabular}{c|c|cccc}
\toprule 
\multicolumn{1}{c|}{\multirow{3}{*}{SSL}}    & \multirow{3}{*}{\shortstack{Priming \\Algorithm}}& \multicolumn{4}{c}{CER/PER} \\ \cline{3-6} 
                         &                             & \multicolumn{2}{c|}{without Adapter}                       & \multicolumn{2}{c}{with Adapter}\\ \cline{3-6} 
                         &                                    & {10m} & \multicolumn{1}{l|}{1h}   & {10m} & {1h}   \\ \midrule
                         \midrule
\multirow{4}{*}{\shortstack[l]{ HuBERT \\ \raggedright (95M)}}  & D-F               & \multicolumn{1}{l}{30.4 }  & \multicolumn{1}{l|}{22.2} & \multicolumn{1}{l}{28.9}  & \multicolumn{1}{l}{20.6}\\  
                         & 1-MTL                   & {32.0}    & \multicolumn{1}{l|}{25.3} & {30.9}  & 23.4 \\  
                          & \cellcolor{FOMAML}MAML & {\cellcolor{FOMAML}29.6} & \multicolumn{1}{l|}{\cellcolor{FOMAML}22.0}   & {\cellcolor{FOMAML}26.2} & \cellcolor{FOMAML}20.4  \\  
                         & \cellcolor{FOMAML}Prime-MTL                                & {\cellcolor{FOMAML}\textbf{29.3}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{21.7}} & {\cellcolor{FOMAML}\textbf{24.6}}  & \cellcolor{FOMAML}\textbf{19.6} \\ \midrule
\multirow{4}{*}{\shortstack[l]{ mHuBERT \\ \raggedright (95M)}} & D-F               & {29.1}  & \multicolumn{1}{l|}{22.0}   & {27.5}  & 19.6 \\  
                         & 1-MTL                   & {31.5}  & \multicolumn{1}{l|}{25.0}   & {29.5}  & 22.5\\  
                         & \cellcolor{FOMAML}MAML                             & {\cellcolor{FOMAML}\textbf{27.7}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}22.2} & {\cellcolor{FOMAML}25.8}  & \cellcolor{FOMAML}\textbf{17.1} \\  
                         & \cellcolor{FOMAML}Prime-MTL                                & {\cellcolor{FOMAML}29.1}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{21.7}}   & {\cellcolor{FOMAML}\textbf{24.1}}  & \cellcolor{FOMAML}19.6 \\ \bottomrule \toprule
\multirow{4}{*}{\shortstack[l]{ XLSR-128 \\ \raggedright (317M)}} & D-F               & {29.8}  & \multicolumn{1}{l|}{21.5} & {25.5}  & 16.6  \\  
                         & 1-MTL                   & {26.4}  & \multicolumn{1}{l|}{19.1} & {20.7}  & 14.6  \\  
                         & \cellcolor{FOMAML}MAML                             & {\cellcolor{FOMAML}25.2}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}18.0}   & {\cellcolor{FOMAML}21.4}  & \cellcolor{FOMAML}13.6  \\  
                         & \cellcolor{FOMAML}Prime-MTL                                & {\cellcolor{FOMAML}\textbf{22.5}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{17.3}} & {\cellcolor{FOMAML}\textbf{18.3}}      &  {\cellcolor{FOMAML}\textbf{13.2}} \\ \bottomrule



\end{tabular}

\end{threeparttable}
% \caption*{ Colored rows refer to our priming baselines. }
% \\``w/o A'' and ``w/ A'' represents without adapter and with adapter cases.}

==> tables/Tune_SSL.tex <==
%\begin{threeparttable} 
%       \captionsetup{justification=raggedright}
%        \captionsetup{font=normal}
% \caption*{For baselines with *, all parameters (including SSL model) are primed/tuned together.\\ The experiment is conducted on Reserve languages track.}
\scalebox{0.75}{
\begin{tabular}{c|c|cc|cc}
\toprule
\multirow{2}{*}{SSL}     & \multirow{2}{*}{\shortstack{Priming \\Algorithm}} & \multicolumn{2}{c|}{CER/PER}      & \multicolumn{2}{c}{STD}   \\ \cline{3-6} 
                         &                                    & \multicolumn{1}{l}{10m} & \multicolumn{1}{l|}{1h}   & \multicolumn{1}{l}{10m} & \multicolumn{1}{l}{1h}   \\ \midrule
\multirow{4}{*}{\shortstack[l]{HuBERT\\ \raggedright (95M)}}  & \multicolumn{1}{l|}{D-F*}              & \multicolumn{1}{l}{29.0}    & \multicolumn{1}{l|}{\textbf{18.4}} & \multicolumn{1}{l}{18.5}  & \multicolumn{1}{l}{8.9}  \\  
 & \multicolumn{1}{l|}{D-F}             & \multicolumn{1}{l}{39.6}    & \multicolumn{1}{l|}{31.3} & \multicolumn{1}{l}{12.3}  & \multicolumn{1}{l}{11.2}  \\

 % & \multicolumn{1}{>{\cellcolor{MTL*}\raggedright}l|}{Prime-MTL*}
  & \multicolumn{1}{l|}{\cellcolor{FOMAML}Prime-MTL*}
                         % &\multicolumn{1}{l}{Prime-MTL*} 
                                         & \multicolumn{1}{l}{\cellcolor{FOMAML}29.3}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}19.0}   & \multicolumn{1}{l}{\cellcolor{FOMAML}19.9}  & \multicolumn{1}{l}{\cellcolor{FOMAML}10.4} \\  
                         & \multicolumn{1}{>{\cellcolor{MTL*}\raggedright}l|}{Prime-MTL}
                         % &\multicolumn{1}{l}{Prime-MTL*} 
                                                                     & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{24.6}}  &\multicolumn{1}{l|}{\cellcolor{FOMAML}19.6} & \multicolumn{1}{l}{\cellcolor{FOMAML}9.7}   &\multicolumn{1}{l}{\cellcolor{FOMAML}8.3}  \\ \midrule
\multirow{4}{*}{\shortstack[l]{ XLSR-128 \\ \raggedright (317M)}} & \multicolumn{1}{l|}{D-F*}              & \multicolumn{1}{l}{19.3}  & \multicolumn{1}{l|}{13.5} & \multicolumn{1}{l}{16.6}  & \multicolumn{1}{l}{16.9} \\  
& \multicolumn{1}{l|}{D-F}             & \multicolumn{1}{l}{32.1}    & \multicolumn{1}{l|}{22.8} & \multicolumn{1}{l}{15.4}  & \multicolumn{1}{l}{13.6}  \\
                         & \multicolumn{1}{>{\cellcolor{MTL*}\raggedright}l|}{Prime-MTL*}
                         % &\multicolumn{1}{l}{Prime-MTL*} 
                                                                           & \multicolumn{1}{l}{\cellcolor{FOMAML}21.2}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}\textbf{12.9}} & \multicolumn{1}{l}{\cellcolor{FOMAML}11.2}  & \multicolumn{1}{l}{\cellcolor{FOMAML}6.9}  \\  
                         & \multicolumn{1}{>{\cellcolor{MTL*}\raggedright}l|}{Prime-MTL}
                         % &\multicolumn{1}{l}{Prime-MTL*} 
                                                                       & \multicolumn{1}{l}{\cellcolor{FOMAML}\textbf{18.3}}  & \multicolumn{1}{l|}{\cellcolor{FOMAML}13.2} & \multicolumn{1}{l}{\cellcolor{FOMAML}8.5}   & \multicolumn{1}{l}{\cellcolor{FOMAML}6.8}  \\ \bottomrule
 
\end{tabular}
}
% \begin{tablenotes}[para,flushleft]    
%         \captionsize         
%         \item Colored rows refer to baselines using our priming pipeline.
%         \item For baselines with *, they prime/tune all parameters (including SSL model) together.
%       \caption*{Colored rows refer to baselines using our priming pipeline.
% \\For baselines with *, they prime/tune all parameters (including SSL model) together.
% \\The experiment is conduct on Reserve languages track.}
%       \end{tablenotes}     


%\end{threeparttable}

==> tables/Update_parameter.tex <==

\scalebox{0.9}{
\begin{tabular}{l|cccc}
\toprule
 \multicolumn{1}{c|}{\multirow{3}{*}{\shortstack{}}} & \multicolumn{4}{c}{CER/PER $\downarrow$} \\ \cmidrule{2-5} 
    XLSR-128   & \multicolumn{2}{c|}{$\theta_a \cup \theta_d$ ($\theta_{a+d}$)}             & \multicolumn{2}{c}{$\theta_s \cup \theta_d$ ($\theta_{s+d}$)} \\ \cmidrule{2-5} 
   & \multicolumn{1}{c|}{10min} & \multicolumn{1}{c|}{1h}   & \multicolumn{1}{c|}{10min}   & 1h     \\ \midrule
 
 \cellcolor{FOMAML}IA-MTL & \multicolumn{1}{c|}{\cellcolor{FOMAML}\textbf{18.3}}  & \multicolumn{1}{c|}{\cellcolor{FOMAML}13.2} & \multicolumn{1}{c|}{\cellcolor{FOMAML}21.2}    & \cellcolor{FOMAML}\textbf{12.9}   \\ \bottomrule
\end{tabular}
}

==> tables/XLSR_table.tex <==
\scalebox{0.8}{\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{3}{*}{Language Track} & \multirow{3}{*}{Priming Algorithm} & \multicolumn{4}{c|}{CER/PER}                                                               & \multicolumn{4}{c}{STD}                                                                   \\ \cline{3-10} 
                                &                                    & \multicolumn{2}{c|}{w/o Adapter}                       & \multicolumn{2}{c|}{w Adapter}    & \multicolumn{2}{c|}{w/o Adapter}                       & \multicolumn{2}{c}{w Adapter}    \\ \cline{3-10} 
                                &                                    & \multicolumn{1}{c|}{10min} & \multicolumn{1}{c|}{1h}   & \multicolumn{1}{c|}{10min} & 1h   & \multicolumn{1}{c|}{10min} & \multicolumn{1}{c|}{1h}   & \multicolumn{1}{c|}{10min} & 1h   \\ \midrule
\multirow{4}{*}{Mono}           & Directly Fine-tuning               & \multicolumn{1}{c|}{39.7}  & \multicolumn{1}{c|}{30.6} & \multicolumn{1}{c|}{32.1}  & 22.8 & \multicolumn{1}{c|}{13.1}  & \multicolumn{1}{c|}{12}   & \multicolumn{1}{c|}{15.4}  & 13.6 \\ \cline{2-10} 
                                & Single-Stage MTL                   & \multicolumn{1}{c|}{54.1}  & \multicolumn{1}{c|}{56.1} & \multicolumn{1}{c|}{51.6}  & 53   & \multicolumn{1}{c|}{17.4}  & \multicolumn{1}{c|}{16.3} & \multicolumn{1}{c|}{19.7}  & 18.4 \\ \cline{2-10} 
                                & FOMAML                             & \multicolumn{1}{c|}{31.5}  & \multicolumn{1}{c|}{24.9} & \multicolumn{1}{c|}{26.4}  & 20   & \multicolumn{1}{c|}{12.2}  & \multicolumn{1}{c|}{11.5} & \multicolumn{1}{c|}{14}    & 12.5 \\ \cline{2-10} 
                                & MTL                                & \multicolumn{1}{c|}{26.3}  & \multicolumn{1}{c|}{20.3} & \multicolumn{1}{c|}{24.1}  & 19.1 & \multicolumn{1}{c|}{13.4}  & \multicolumn{1}{c|}{12.3} & \multicolumn{1}{c|}{13.4}  & 12   \\ \midrule
\multirow{4}{*}{Reserve}        & Directly Fine-tuning               & \multicolumn{1}{c|}{29.8}  & \multicolumn{1}{c|}{21.5} & \multicolumn{1}{c|}{25.5}  & 16.6 & \multicolumn{1}{c|}{19.7}  & \multicolumn{1}{c|}{16.4} & \multicolumn{1}{c|}{21}    & 16   \\ \cline{2-10} 
                                & Single-Stage MTL                   & \multicolumn{1}{c|}{26.4}  & \multicolumn{1}{c|}{19.1} & \multicolumn{1}{c|}{20.7}  & 14.6 & \multicolumn{1}{c|}{9.1}   & \multicolumn{1}{c|}{7.5}  & \multicolumn{1}{c|}{7.9}   & 6.1  \\ \cline{2-10} 
                                & FOMAML                             & \multicolumn{1}{c|}{25.2}  & \multicolumn{1}{c|}{18}   & \multicolumn{1}{c|}{21.4}  & 13.6 & \multicolumn{1}{c|}{14.4}  & \multicolumn{1}{c|}{8}    & \multicolumn{1}{c|}{15.7}  & 6.9  \\ \cline{2-10} 
                                & MTL                                & \multicolumn{1}{c|}{22.5}  & \multicolumn{1}{c|}{17.3} & \multicolumn{1}{c|}{18.3}  & 13.2 & \multicolumn{1}{c|}{9.2}   & \multicolumn{1}{c|}{7.6}  & \multicolumn{1}{c|}{8.5}   & 6.8  \\ \bottomrule
\end{tabular}}
